Differentially Private Testing of Identity and Closeness of Discrete Distributions

We study the fundamental problems of identity testing (goodness of fit), and closeness testing (two sample test) of distributions over $k$ elements, under differential privacy. While the problems have a long history in statistics, finite sample bounds for these problems have only been established recently. In this work, we derive upper and lower bounds on the sample complexity of both the problems under $(\varepsilon, \delta)$-differential privacy. We provide optimal sample complexity algorithms for identity testing problem for all parameter ranges, and the first results for closeness testing. Our closeness testing bounds are optimal in the sparse regime where the number of samples is at most $k$. Our upper bounds are obtained by privatizing non-private estimators for these problems. The non-private estimators are chosen to have small sensitivity. We propose a general framework to establish lower bounds on the sample complexity of statistical tasks under differential privacy. We show a bound on differentially private algorithms in terms of a coupling between the two hypothesis classes we aim to test. By constructing carefully chosen priors over the hypothesis classes, and using Le Cam's two point theorem we provide a general mechanism for proving lower bounds. We believe that the framework can be used to obtain strong lower bounds for other statistical tasks under privacy.

==> binary-lower.tex <==
\subsection{Lower Bound for Binary Testing}

Firstly, let us consider the lower bound. Without loss of generality, we consider distinguishing between $\mathcal{P} \sim Bern(\frac1{2}-\alpha)$, and $\mathcal{Q} \sim Bern(\frac1{2}+\alpha)$. Then we can have the following lemma:

\begin{lemma}
	\label{resamp_binary}
	Given sample access to an unknown Bernoulli distribution $p$. If there exists an $\epsilon$-differentially private algorithm $\mathcal{A}_1$which distinguishes between $p = \mathcal{P}$ and $p = \mathcal{Q}$ with probability $1 - \gamma$ using $m$ samples. Then there exists an algorithm $\mathcal{A}_2$, which takes only $\phi_1$ as input and can achieve the same accuracy while satisfying that:
	\begin{equation}
	 e^{-\epsilon \alpha m} \leq \frac{P[\mathcal{A}_2(\phi_1 = \frac{m+\alpha m }{2}) = \mathcal{Q}]}{P[\mathcal{A}_2(\phi_1 = \frac{m-\alpha m }{2}) = \mathcal{Q}]} \leq e^{\epsilon \alpha m}.
	\end{equation}
	where $\phi_1$ is the number of 1s which appear in the sample.
\end{lemma}

\textit{Proof of lemma~\ref{resamp_binary}}

Given an algorithm $\mathcal{A}_1(\bar{x})$ using sample sequence as inputs, we consider the following algorithm which only has access to $\phi_1$,
\begin{itemize}
	\item[1] Resample $\bar{y}$ uniformly from the sequences where symbol 1 appear $\phi_1$ times in the sample.
	\item[2] Return $\mathcal{A}_1(\bar{y})$.
\end{itemize}

Then this algorithm satisfies the constraints in lemma~\ref{resamp_binary}. For accuracy,

\begin{align}
P_e(\mathcal{A}_2) = \sum_{\phi_1} P_e(\mathcal{A}_2 | \phi_1) P(\phi_1) = \sum_{\phi_1} P(\phi_1) \sum_{\bar{y} \sim \phi_1} P_e(\mathcal{A}_1(\bar{y})) P(\bar{y} | \phi_1)\\
= \sum_{\phi_1}  \sum_{\bar{y} \sim \phi_1} P_e(\mathcal{A}_1(\bar{y})) \frac{P(\phi_1)}{\# \{\phi_1\}} = \sum_{\phi_1}  \sum_{\bar{y} \sim \phi_1} P_e(\mathcal{A}_1(\bar{y})) P(\bar{y})\\
= \sum_{\bar{y}} P_e(\mathcal{A}_1(\bar{y})) P(\bar{y}) = P_e(\mathcal{A}_1)
\end{align}

For privacy condition, we consider the following matching scheme,

All the nodes in the graph are sequences whose $\phi_1 =  \frac{m-\alpha m }{2} $ or $\phi_1 =  \frac{m+\alpha m }{2}$. We denote them by $A$ and $B$. A sequence $\bar{x}$ from $A$ are connected to a sequence $\bar{y}$ from $B$ if and only if by changing only $\alpha m$ samples in $\bar{x}$ we can get $\bar{y}$. Then we know the number of nodes in $A$ and $B$ are both $m \choose \frac{m-\alpha m}{2}$. And each node in $A$ or $B$ is connected to $\frac{m+\alpha m}{2} \choose \alpha m$ nodes in $B$ or $A$. So the graph is a regular bipartite graph. Then it must have a perfect matching.  

Suppose the match is $f: \bar{B} \rightarrow \bar{A}$. Then by differential privacy:
\begin{equation}
\forall \bar{x} \in \bar{B}, e^{-\epsilon \alpha m} \leq \frac{P[\mathcal{A}_1(\bar{x}) = \mathcal{Q}]}{P[\mathcal{A}_1(f(\bar{x})) = \mathcal{Q}]} \leq e^{\epsilon \alpha m}
\end{equation}

Hence we have:
\begin{align}
&P[\mathcal{A}_2(\phi_1 = \frac{m+\alpha m }{2}) = \mathcal{Q}] \\
= &\sum_{\bar{x} \in \bar{B} } P[\mathcal{A}_1(\bar{x}) = \mathcal{Q}] P[\bar{x}]  \\
= &\frac{\sum_{\bar{x} \in \bar{B}} P[\mathcal{A}_1(\bar{x}) = \mathcal{Q}]}{\# \{\phi_1 = \frac{m+\alpha m }{2} \} }   
\leq \frac{ \sum_{\bar{x} \in \bar{B}} e^{\epsilon \alpha m} P[\mathcal{A}_1(f(\bar{x})) = \mathcal{Q}]}{ \# \{\phi_1 = \frac{m+\alpha m }{2}\} } \\
= & e^{\epsilon \alpha m} \frac{ \sum_{\bar{y} \in \bar{A}} P[\mathcal{A}_1(\bar{y}) = \mathcal{Q}]}{\# \{\phi_1 = \frac{m-\alpha m }{2} \} } \\ 
= & e^{\epsilon \alpha m} \sum_{\bar{x} \in \bar{A}} P[\mathcal{A}_1(\bar{x}) = \mathcal{Q}] P[\bar{x}]
 \\=& e^{\epsilon \alpha m} P[\mathcal{A}_2(\phi_1 = \frac{m-\alpha m }{2}) = \mathcal{Q}]
\end{align}

Similarly, we can prove the other side of the inequality.

Hence we have proved lemma~\ref{resamp_binary}.

Then we consider the upper bound of the Binary Hypothesis Testing problem.

\textit{Proof of Theorem~\ref{lower_bina} }:

$m = \Omega(\frac1{\alpha^2})$ has been proved in the previous literature. Now we prove that $m = \Omega(\frac1{\alpha \epsilon})$. By lemma~\ref{resamp_binary}, we know that we only need to prove if $m = \Omega(\frac1{\alpha \epsilon})$, there is no algorithm $\mathcal{A}$ that takes $\phi_1$ as input and can achieve an accuracy of $0.6$ in distinguishing $\mathcal{P}$ and $\mathcal{Q}$. WLOG, we assume the prior probability of $\mathcal{P}$ and $\mathcal{Q}$ are both $1/2$. So the error probability is:

\begin{align}
	P_e \geq &\frac{1}{2} P[|\phi_1 - \frac{m+\alpha m}{2}| < 10 \sqrt{Var_{\mathcal{Q}}(\phi_1)} | \mathcal{Q}] P[\mathcal{A}(\frac{m+\alpha m}{2} + 10 \sqrt{Var_{\mathcal{Q}}(\phi_1)}) = \mathcal{P}] \\
	&+ \frac{1}{2} P[|\phi_1 - \frac{m-\alpha m}{2}| < 10 \sqrt{Var_{\mathcal{P}}(\phi_1)} | \mathcal{P}] P[\mathcal{A}(\frac{m-\alpha m}{2} -10 \sqrt{Var_{\mathcal{P}}(\phi_1)}) = \mathcal{Q}]  \\
	\geq &  \frac{1}{2} 0.99 (1-q_1)+\frac{1}{2} 0.99 q_2 \\
	\geq &\frac{1}{2} 0.99 (q_2 + 1- q_2 e^{\epsilon(\alpha m+ 10 \sqrt{Var_{\mathcal{Q}}(\phi_1)} + 10 \sqrt{Var_{\mathcal{P}}(\phi_1))}})
\end{align}
where $q_1 = P[\mathcal{A}(\frac{m+\alpha m}{2} + 10 \sqrt{Var_{\mathcal{Q}}(\phi_1)}) = \mathcal{Q}]$, and $q_2 = P[\mathcal{A}(\frac{m-\alpha m}{2} -10 \sqrt{Var_{\mathcal{P}}(\phi_1)}) = \mathcal{Q}] $

Hence if $m = o(\frac1{\alpha \epsilon})$,
\begin{equation}
	P_e \geq \frac{1}{2} 0.99 (q_2 + 1- q_2) = \frac{1}{2} 0.99 \geq 0.4
\end{equation}

which proves the theorem.



==> binary.tex <==


\subsection{Varied arguments for the same thing}

We now provide a $\eps$-differentially private algorithm for testing whether $\p = \Bern{\bias_0}$, or $\p = \Bern{\bias}$, for some $\bias$ such that $\absv{\bias_0-\bias}\ge\alpha$. The sample complexity of the algorithm is $O\Paren{\frac1{\alpha^2}+\frac1{\alpha\eps}}$.

Consider the following statistics:
$$ Z(D) = \frac1{m \alpha} (\phi_1 - \bias_0 m)$$
where $\phi_1$ is the number of 1s which appear in the sample. 

As proved in the previous literature, $E[Z]=0$ when $\bias=\bias_0$ and $\absv{E[Z]} \ge 1 $ when $\absv{\bias-\bias_0}\ge\alpha$, and the variance of Z is such that these two cases can be separated constant probability. A natural approach to make it differentially private is to truncate this statistics into range $[0,1]$, and interpret it as the probability of the output.  If $\bias=\bias_0$, the result is likely to be $0$ and if $\absv{\bias-\bias_0}\ge\alpha$, the result is likely to be 1. This statistics is naturally private because it has a low sensitivity. The pseudocode for the algorithm is provided in Algorithm \ref{algorithm_binary}.


\begin{algorithm}
    \caption{}
    \label{algorithm_binary}
    \hspace*{\algorithmicindent} \textbf{Input:}
    $\epsilon$, $\alpha$, $\bias_0$, sample access to distribution $p$
    \begin{algorithmic}[1] 
    \State Sample $X \sim Bernoulli (1/5)$
    \If{X = 1} \\
    ~~~~\Return $\absv{\bias-\bias_0}=0$ or $\absv{\bias-\bias_0}\ge\alpha$ with the same probability.
    \Else 
    \State Let $\phi_1$ denotes the number of 1s which appear in the sample.
    \State $Z \gets \frac1{m \alpha} (\phi_1 - \bias_0 m)$
    \State Let $T$ be the closest value to $\absv{Z}$ in the interval in $[0,1]$
    \State Sample $Y \sim Bernoulli (T)$
    \If{Y=1} \\
    ~~~~~~~~\Return $\absv{\bias-\bias_0}\ge\alpha$
    \Else \\
     ~~~~~~~~\Return $\absv{\bias-\bias_0}=0$
    ~~~~\EndIf
    \EndIf     
\end{algorithmic}
\end{algorithm}

\begin{theorem}
Algorithm~\ref{algorithm_binary} is an $\eps$-differentially private algorithm for testing if a binary distribution is $\Bern{\bias_0}$. Moreover, it has error probability at most $1/3$, with sample complexity $O\Paren{\frac1{\alpha^2}+\frac1{\alpha\eps}}$.
\end{theorem}

We proceed to prove the two aspects of the algorithm, correctness and privacy.

First we consider the correctness. We have the following two lemmas, which rely on the condition that $m = \Omega (\frac1{\alpha^2})$.

\begin{lemma}
	\label{correctness_expec_binary}
	Given $\bias = \bias_0$, $E(Z) = 0$. Given $\absv{\bias-\bias_0}\ge\alpha$, $\absv{E(Z)} \ge 1$.
\end{lemma}

\textit{Proof of lemma~\ref{correctness_expec_binary}}

Given $\bias = \bias_0$, 
$$\mathbf{E}(Z) = \frac1{m\alpha} \Paren{ \mathbf{E}(\phi_1) - \bias_0m }  = 0 $$

Given $\absv{\bias-\bias_0}\ge\alpha$, $\absv{E(Z)} \ge 1$.
$$\absv {\mathbf{E}(Z)} = \frac1{m\alpha} \absv{ \mathbf{E}(\phi_1) - \bias_0m }  =  \frac1{\alpha} \absv{\bias-\bias_0} \ge 1$$

\begin{lemma}
	\label{correctness_variance_binary}
	Given $\bias = \bias_0$, $\mathbf{Var}(Z) \le \frac1{1000}$. Given $\absv{\bias-\bias_0}\ge\alpha$, $\mathbf{Var}(Z) \le \frac1{1000} \mathbf{E}^2(Z)$.
\end{lemma}

\textit{Proof of lemma~\ref{correctness_variance_binary}}

To be filled.

We consider the case $\bias = \bias_0$. According to Chebyshev's inequality, we get that $Z \le 1/10$ with probability at least $9/10$, and we output  $\bias = \bias_0$ with probability $1/10+4/5*(9/10)^2 \ge 2/3$ . Similarly, when $\absv{\bias-\bias_0}\ge\alpha$, $\absv{E(Z)} \ge 1$, $Z \ge 9/10$ with probability at least $9/10$, and we get the right answer with probability greater than $2/3$. 

Then we consider the privacy. We will prove the algorithm is $(0,\frac1{10} \epsilon)$ differentially private. Because each output for the algorithm is at least $1/10$, so the $(0,\frac1{10} \epsilon)$ differential privacy will imply $(\epsilon,0)$ differential privacy.

Now we consider the value of $T$ for two neighboring datasets $D$ and $D ^ \prime$, where  $D ^ \prime$ has one fewer occurrence of sample.

\begin{align}
\absv{T(D) - T(D^\prime)} \le &\absv{Z(D)-Z(D^\prime)} \\
\leq& \frac1{m\alpha} \absv{ \phi_1(D) - \phi_1(D ^\prime)} \\
\leq& \frac1{m\alpha} 
\end{align}

When $m = O( \frac1{ \alpha \epsilon})$, $\absv{T(D) - T(D^\prime)} \le \frac1{8} \epsilon $. Suppose the output is $\bias = \bias_0$, the difference of the output probability for $D$ and $D^\prime$ is at most $4/5 * \absv{T(D)- T(D^\prime)} \le \frac1{10} \epsilon$. And things are similar if we output $\absv{\bias-\bias_0}\ge\alpha$. So we have proved our algorithm is $(0,\frac1{10} \epsilon)$. Combining with the previous argument, the algorithm is also $(\epsilon,0)$ differentially private.








==> coupling-binomial.tex <==
\section{Coupling of maximum of two Binomial Distributions}

Let $0\le r\le 1$, and suppose $X\sim{\rm Bin}(n,r)$. Then, the cumulative density function (CDF) of $X$ for a $k$ is $F(t,p) = \probof{X\le t}= \sum_{i=0}^{k}{n\choose i}r^i(1-r)^{n-i}$. Then $F(t,r)$ as a function of $r$ for a fixed $t$ is log-concave. This result follows from the log-concavity of incomplete Beta Functions, which we state for completeness.
\begin{lemma}
	For a fixed $t$, $F(t,r)$ is log-convex in $r$. \label{lem:log-concave-cdf}
\end{lemma}
\begin{proof}
	Note that 
	\begin{align}
		F(t,r) = \sum_{i=0}^{\lfloor t\rfloor}{n\choose i}r^i(1-r)^{n-i} = I_{1-r}(n-t, t+1),
	\end{align}
	where 
	\[
	I_x(a,b) = \frac{{\int_{0}^{x} u^{a-1}{(1-u)}^{b-1}du}}{\int_{0}^{1} u^{a-1}{(1-u)}^{b-1}du}
	\]
	is the incomplete regularized beta function. This is the CDF of a beta distribution. Using the fact that beta distribution is log-concave, and the CDF of a log-concave distribution is log-concave. Therefore, $I_x(a,b)$ is log-concave. This also imples that $I_{1-x}(a,b)$ is log-concave, implying that $F(t,r)$ is log-concave.
\end{proof} 

\begin{definition}
	A random variable $Y_1$ is said to stochastically dominate $Y_2$ if $\probof{Y_1\ge t}\ge \probof{Y_2\ge t}$ for any $x$. 
\end{definition}

\begin{definition}
	A coupling $Y_1'$, $Y_2'$ is a monotone coupling if $\probof{Y_1'\ge Y_2'}=1$. 
\end{definition}
\cite{???}
\begin{lemma}
	$Y_1$ stochastically dominate $Y_2$ if and only if there is a monotone coupling between $Y_1$, and $Y_2$.
\end{lemma}

As a corollary we obtain, 
\begin{lemma}
	Suppose $Y_1'$, $Y_2'$ is a monotone coupling of $(Y_1, Y_2)$. Then, $\expectation{Y_1'}-\expectation{Y_2'}= \expectation{Y_1}-\expectation{Y_2}$. 
\end{lemma}

We will now discuss coupling of maximum of Binomial distributions. Let $0<\alpha\le1/2$. Suppose $X_1\sim{\rm Bin}(n,\frac{1+\alpha}2)$, and $X_2\sim{\rm Bin}(n,\frac{1-\alpha}2)$ are Binomial distributions. Let $X(\alpha)=\max\{X_1, X_2\}$ be the random variable that is the maximum of the two binomials. Note that for any $\alpha>0$, $X_1+X_2$ is $\sim{\rm Bin}(2n,\frac12)$, independent of $\alpha$. 

\begin{lemma}
	Let $\alpha_1>\alpha_2>0$, then $X(\alpha_1)$ stochastically dominates $X(\alpha_2)$. 
\end{lemma}
\begin{proof}
	For any $t$, 
	\begin{align}
		\probof{X(\alpha_1)> t} & = 1- \probof{\max\{X_1, X_2\}\le t} \\
		& = 1-\probof{X_1\le t \text{ and } X_2\le t}\\
		& = 1 - F\left(t, \frac{1+\alpha_1}2\right) F\left(t, \frac{1-\alpha_1}2\right).
	\end{align}
	By Lemma~\ref{lem:log-convex-cdf}, $F\left(t, r\right)$ is log-concave. Therefore, 
	\[
	F\left(t, \frac{1+\alpha_1}2\right) F\left(t, \frac{1-\alpha_1}2\right)
	\le  F\left(t, \frac{1+\alpha_2}2\right) F\left(t, \frac{1-\alpha_2}2\right).
	\]
	This proves that $\probof{X(\alpha_1)\ge t}\ge \probof{X(\alpha_2)\ge t}$, proving the stochastic dominance result. 
\end{proof}












==> uniformity-upper_new.tex <==
\subsection{Identity Testing -- Upper Bounds} \label{sec:upper-uniformity}

We had mentioned in the results that we can use the statistic of Paninski~\cite{Paninski08} to achieve the optimal sample complexity in the sparse case. This result is shown in Section~\ref{??}. We will show that by privatizing the statistic proposed in~\cite{diakonikolas2017sample} we can achieve the sample complexity in Theorem~\ref{thm:main-identity} for all parameter ranges. The procedure is described in Algorithm~\ref{algorithm_uniformity}.

%By the previous argument, any upper bound on uniformity testing is a bound on identity testing. To obtain differentially private algorithms, we need test statistic with small sensitivity. With these arguments, we propose Algorithm~\ref{algorithm_uniformity} for uniformity testing.

%\begin{theorem}
%\label{thm:upper}
%Algorithm~\ref{algorithm_uniformity} achieves an upper bound of 
%\[
%    \Sitd =
%    \begin{cases}
%                                   \Theta\Paren{\frac{\sqrt k}{\alpha^2} + \frac{\ab^{1/2}}{\alpha(\eps+\delta)^{1/2}}}, & \text{when $m \le k$} \\
%                                   \Theta\Paren{\frac{\sqrt k}{\alpha^2} +\frac{\ab^{1/3}}{\alpha^{4/3}(\eps+\delta)^{2/3}}}, & \text{when $k< m \le \frac{k}{\alpha^2}$} \\
%                                   \Theta\Paren{\frac{\sqrt k}{\alpha^2} + \frac1{\alpha \eps+\delta}} & \text{when  $m \ge \frac{k}{\alpha^2}$.  } 
%    \end{cases}
%\]
%We can combine the three bounds to obtain 
%\[
%\Sitd = \Theta\Paren{\frac{k^{1/2}}{\dist^2}+\max\left\{\frac{\ab^{1/2}}{\alpha(\eps+\delta)^{1/2}}, \frac{\ab^{1/3}}{\alpha^{4/3}(\eps+\delta)^{2/3}}, \frac1{\dist(\eps+\delta)}\right\}}.
%\] 
%\end{theorem}


Recall that $\Mltsmb{\smb}{\Xon}$ is the number of appearances of $\smb$ in $\Xon$. Let
\[
S(\Xon) \ed\sum_{x=1}^{n} \absv{ \frac {\Mltsmb{\smb}{\Xon} } {m} -\frac1{k} },
\]
be the distance of the empirical distribution from the uniform distribution. Let $\mu(p) = \expectation{S(\Xon)}$ when the samples are drawn from distribution $p$. They show the following separation result on the expected value of $S(\Xon)$. 
\begin{lemma}[\cite{diakonikolas2017sample}]
Let $p$ be a distribution over $[n]$ and $\alpha = \dtv{\p}{\unifab}$, then there is a constant $c$ such that 
$$ \mu(\p) - \mu (\unifab) \ge  \left\{
\begin{array}{lll}

c{\alpha^2 \cdot  \frac{m^2}{k^2}},    &      & \text{when $m<k$}\\
c{\alpha^2 \cdot \sqrt { \frac{m}{k} }},  &      &  \text{when $k< m \le \frac{k}{\alpha^2}$} \\
c{\alpha},       &      & \text{when $~ m \ge \frac{k}{\alpha^2}$ }
\end{array} \right. $$\label{lem:diako}
\end{lemma}

\cite{diakonikolas2017sample} used this result to show that thresholding $S(\Xon)$ at 0 is an optimal algorithm for identity testing. Their result is stronger than what we require in our work, since we only care about making the error probability at most 0.1. We first normalize the statistic to simplify the presentation of our DP algorithm. Let
\begin{equation}\label{eqn:statistic}
    Z (\Xon) \ed
    \begin{cases}
                                   k \Paren {S(\Xon) - \mu (\unifab) - \frac1{2} c \alpha^2 \cdot  \frac{m^2}{k^2} ~}, & \text{when $m \le k$} \\
                                   m \Paren {S(\Xon) - \mu (\unifab) - \frac1{2} c \alpha^2 \cdot \sqrt { \frac{m}{k} } ~}, & \text{when $k< m \le \frac{k}{\alpha^2}$} \\
                                   m \Paren {S(\Xon) - \mu (\unifab)  - \frac1{2} c \alpha}, & \text{when  $m \ge \frac{k}{\alpha^2}$  } 
    \end{cases}
\end{equation}
where $c$ is the constant in Lemma~\ref{lem:diako}, and $\mu(\unifab)$ is the expected value of  ${S(\Xon)}$ when $\Xon$ are drawn from uniform distribution.

Therefore, for $\Xon$ from $\unifab$, 
\begin{equation}\label{eqn:statistic-expectation-uniform}
    \expectation{Z (\Xon)} \le
    \begin{cases}
                                   - \frac1{2} c \alpha^2 \cdot  \frac{m^2}{k}, & \text{when $m \le k$} \\
                                    - \frac1{2} c \alpha^2 \cdot  { \frac{m^{3/2}}{k^{1/2}} }, & \text{when $k< m \le \frac{k}{\alpha^2}$} \\
                                  -\frac1{2} cm \alpha, & \text{when  $m \ge \frac{k}{\alpha^2}$  } 
    \end{cases}
\end{equation}

When $\Xon$ is drawn from $\p$ with $\dtv{\p}{\unifab}\ge\alpha$, 
\begin{equation}\label{eqn:statistic-expectation-far}
    \expectation{Z (\Xon)} \ge
    \begin{cases}
                                   \frac1{2} c \alpha^2 \cdot  \frac{m^2}{k}, & \text{when $m \le k$} \\
                                    \frac1{2} c \alpha^2 \cdot  { \frac{m^{3/2}}{k^{1/2}} }, & \text{when $k< m \le \frac{k}{\alpha^2}$} \\
                                  \frac1{2} c m\alpha, & \text{when  $m \ge \frac{k}{\alpha^2}$  } 
    \end{cases}
\end{equation}

%%%%%%%%
\iffalse
When  $k < m \le \frac{k}{\alpha^2}$, suppose $\Xon\sim\p$, then
\[
\expectation{Z(\Xon)} = - \frac1{2} c m \alpha^2 \cdot \sqrt { \frac{m}{k} }, \text{ if $\p=\unifab$},
\]
and $\Xon\sim\p$, 
\[
\expectation{Z(\Xon)} \ge  \frac1{2}c m \alpha^2 \cdot \sqrt { \frac{m}{k} }, \text{if $\dtv{\p}{\unifab}\ge\dist$}. 
\]

When  $m \ge \frac{k}{\alpha^2}$, suppose $\Xon\sim\p$, then
\[
\expectation{Z(\Xon)} = - \frac1{2} c m \alpha, \text{ if $\p=\unifab$},
\]
and $\Xon\sim\p$, 
\[
\expectation{Z(\Xon)} \ge  \frac1{2} c m  \alpha, \text{if $\dtv{\p}{\unifab}\ge\dist$}. 
\]
\fi
%%%%%%%%
%%%%%%%
\iffalse
\begin{algorithm}
\textbf{Input:} $\eps$, $\dist$, i.i.d. samples $\Xon$ from $\p$\\
\textbf{Output:} 1 if $\p= \unif$, 0 otherwise \\
If $  Z(\Xon) \le 0$\\
\quad \textbf{return} a $\Bern{0.5 e^{\eps Z(\Xon)}}$ random variable, \\
else \\
\qquad \textbf{return} a $\Bern{1-0.5 e^{-\eps Z(\Xon)}}$ random variable.
\label{alg:bernoulli-identity}
\caption{Testing a fair coin}
\end{algorithm}


We modify their algorithm slightly to obtain a differentially private algorithm. Let 
\[
Z(\Xon) =  \frac{\ns^2\alpha^2}{2\ab} \Brack{ \ns\cdot\Paren{1-\frac1\ab}^{\ns-1} - \prfsmb{1}{\Xon} }
\]
Then we get the following algorithm.
\fi
%%%%%%%%

\begin{algorithm}
    \caption{Uniformity testing}
    \label{algorithm_uniformity}
    \hspace*{\algorithmicindent} \textbf{Input:}  $\eps$, $\dist$, i.i.d. samples $\Xon$ from $\p$
    \begin{algorithmic}[1] 
    \State Define the random variable $S(\Xon) = \frac1{2} \sum_{x=1}^{n} \absv{ \frac {\Mltsmb{\smb}{\Xon} } {m} -\frac1{k} }$
    \State Let $Z(\Xon)$ be evaluated from~\eqref{eqn:statistic}.
    ~~~~~~~~
    \State Generate $Y\sim\Bern{\sigma\Paren{\eps\cdot Z}}$, $\sigma$ is the sigmoid function.
    \If{$Y=0$}
    \State {\Return $\p=\unifab$}
    \Else 
    \State {\Return $\p\ne \unifab$}
    \EndIf
\end{algorithmic}
\end{algorithm}


Before proving the privacy bounds, we prove the following (weak) version of the result of~\cite{diakonikolas2017sample}, which is sufficient to prove the sample complexity bound   for constant error probability
\begin{lemma}
There is a constant $C>0$, such that when $\ns>C\sqrt{\ab}/\dist^2$, then for $\Xon$ from $\unifab$
\[
\probof{Z(\Xon)>\frac{\expectation{Z(\Xon)}}3} <0.01,
\]
and for $\p$ with $\dtv{\p}{\unifab}\ge\alpha$,
\[
\probof{Z(\Xon)<\frac{\expectation{Z(\Xon)}}3} <0.01.
\]
\end{lemma}


We first prove the privacy bound. When $m \ge k$, if we change  one symbol in $\Xon$, $S(\Xon)$ can change by at most $1/m$. So $Z(\Xon)$ can change at most 1. Else when $m<k$, \cite{diakonikolas2017sample} also shows that  $S(\Xon)$ can change by at most $1/k$ when we change one symbol in  $\Xon$. So $Z(\Xon)$ can also change at most 1. Therefore $\eps\cdot Z$ changes by at most $\eps$. Invoking Lemma~\ref{lem:sig-cont}, the probability of any output changes by a multiplicative $\exp(\eps)$, and the algorithm is $\eps$-differentially private.

Then we consider the proof for the error probability. In order to get our result, we need the following lemma, which is proved in \cite{diakonikolas2017sample}.
\begin{lemma}{(Bernstein version of McDiarmid's inequality)}
\label{lem:McDiarmid}
	Let $\Yon$ be independent random variables taking values in the set $\cY$. Let $f: \cY^m \rightarrow \RR$ be a function of $\Yon$ so that for every $j \in [m]$, and $y_1,...y_m,{y_j \prime} \in \cY$, we have that:
$$\absv{f(y_1,...y_j,...y_m) - f(y_1,...,{y_j \prime},...y_m)} \le B $$,

Then we have

$$\probof{f-\expectation{f} \ge z} \le \exp(\frac{-2z^2}{mB^2})$$.

In addition, if for each $j \in [m]$ and $y_1,...y_{j-1},y_{j+1},...y_m$ we have that 

$$ \mathrm{Var}_{Y_j} [f(y_1,...y_j,...y_m)] \le \sigma_j^2$$,

then we have 
$$\probof{f-\expectation{f} \ge z} \le \exp(\frac{-z^2}{\sum_{j=1}^{m} \sigma_j^2 +2Bz/3 })$$.
\end{lemma}


We first consider the case when $k< m \le \frac{k}{\alpha^2}$. When $p=\unifab$, we get $\expectation{Z(\Xon)} = - \frac1{2} c m \alpha^2 \cdot \sqrt { \frac{m}{k} }$, then by the first part of Lemma~\ref{lem:McDiarmid},
 \begin{align}
\probof{Z(\Xon)> -   \frac1{6} c m \dist^2 \cdot \sqrt{\frac{m}{k}}}   \le& 
\probof{Z(\Xon) - \expectation{Z(\Xon) } > \frac{2}{3}c m \dist^2 \cdot \sqrt{\frac{m}{k}}} \nonumber\\
\le & \exp( -\frac{4c^2m^2 \dist^4}{9k} )
\end{align}

Therefore, there is a $C_1$ such that if $\ns\ge C_1\sqrt{\ab}/\alpha^2$, then under the uniform distribution $\probof{Z(\Xon)> - \frac1{6} c m \dist^2 \cdot \sqrt{\frac{m}{k}}} $ is at most 1/100. Now furthermore, if $\eps c \cdot m \dist^2 \cdot \sqrt{\frac{m}{k}}>\log(25)$, then for all $\Xon$ with $Z(\Xon)<-   \frac1{6} c m \dist^2 \cdot \sqrt{\frac{m}{k}} $, with probability at least 0.95, the algorithm outputs the uniform distribution. Combining the conditions, we obtain that there is a constant $C_2$ such that for $\ns = C_2\Paren{\frac{\sqrt{\absz}}{\alpha^2}+ \frac{ k^{ 1/3 } } { \alpha^{4/3}  \eps^{ 2/3 } }}$, with probability at least 0.9, the algorithm outputs uniform distribution when the input distribution is indeed uniform.  We also omit the case of non-uniform distribution part because of the same reason.

Then we consider the case when $\frac{k}{\alpha^2} < m$. When $p=\unifab$, we get $\expectation{Z(\Xon)} = - \frac1{2} c m \alpha$, then by the Bernstein version of McDiarmid's inequality,
 \begin{align}
\probof{Z(\Xon)> -   \frac1{6} c m \dist}    \le& 
\probof{Z(\Xon) - \expectation{Z(\Xon) } > \frac{2}{3}c m \dist } \nonumber\\
\le & \exp( -\frac{4c^2m \dist^2}{9} )
\end{align}

Using the same argument we can show that there is a constant $C_2$ such that for $\ns = C_2\Paren{\frac{\sqrt{\absz}}{\alpha^2}+ \frac1{\alpha \eps}}$, with probability at least 0.9, the algorithm outputs uniform distribution when the input distribution is indeed uniform. The case of non-uniform distribution is similar since the variance bounds hold for both the cases, and is omitted. 

%%%%%%%%
\iffalse
Therefore, there is a $C_1$ such that if $\ns\ge C_1/\alpha^2$, then under the uniform distribution $\probof{Z(\Xon)>-\frac{c \ns \dist}{6}}$ is at most 1/100. Now furthermore, if $\eps \cdot c m \dist>\log(25)$, then for all $\Xon$ with $Z(\Xon)<-\frac{c\ns\dist}{6}$, with probability at least 0.95, the algorithm outputs the uniform distribution. Combining the conditions, we obtain that there is a constant $C_2$ such that for $\ns = C_2\Paren{\frac{\sqrt{\absz}}{\alpha^2}+ \frac1{\alpha \eps}}$, with probability at least 0.9, the algorithm outputs uniform distribution when the input distribution is indeed uniform.The case of non-uniform distribution is similar since the variance bounds hold for both the cases, and is omitted.
\fi
%%%%%%%%

At last we consider the case when $m \le k$. This case is a little different. When $p=\unifab$, we get $\expectation{Z(\Xon)} = - \frac1{2} c k \alpha^2 \cdot \frac{m^2}{k^2}$, then by the second part of Lemma~\ref{lem:McDiarmid},
 \begin{align}
\probof{Z(\Xon)> -   \frac1{6} c \dist^2 \cdot \frac{m^2}{k}}   \le& 
\probof{Z(\Xon) - \expectation{Z(\Xon) } > \frac{2}{3}c  \dist^2 \cdot \frac{m^2}{k}} \nonumber\\
\le & \exp( \frac{-\frac{4}{9}c^2 \dist^4 \frac{m^4}{k^2} }{ \frac{m^2}{k} + \frac{4}{9}c \dist^2 \frac{m^2}{k}} ) \\
\le & \exp(-\frac{2}{9}c \alpha^4 \frac{m^2}{k})
\end{align}
The last inequality comes from the fact that for any $j$, the variance of $Z$ as $Y_j$ varies and the other $Y_{j \prime}$'s are kept is smaller than $m/k$, which is proved in  \cite{diakonikolas2017sample} and then we can use the second part of  Lemma~\ref{lem:McDiarmid}.

Therefore, there is a $C_1$ such that if $\ns\ge C_1\sqrt{\ab}/\alpha^2$, then under the uniform distribution $\probof{Z(\Xon)> - \frac1{6} c k \dist^2 \cdot \frac{m^2}{k^2}} $ is at most 1/100. Now furthermore, if $\eps c \cdot k \dist^2 \cdot \frac{m^2}{k^2}>\log(25)$, then for all $\Xon$ with $Z(\Xon)<-   \frac1{6} c k \dist^2 \cdot \frac{m^2}{k^2} $, with probability at least 0.95, the algorithm outputs the uniform distribution. Therefore, we obtain that there is a constant $C_2$ such that for $\ns = C_2\Paren{\sqrt{\ab}/\alpha^2+\frac{\sqrt{k}}{\alpha \sqrt{\eps}}}$, with probability at least 0.9, the algorithm outputs uniform distribution when the input distribution is indeed uniform. The case of non-uniform distribution is similar and is omitted. 




